Improving Pixel-based MIM by Reducing Wasted Modeling Capability

There has been significant progress in Masked Image Modeling (MIM). Existing MIM methods can be broadly categorized into two groups based on the reconstruction target: pixel-based and tokenizer-based approaches. The former offers a simpler pipeline and lower computational cost, but it is known to be biased toward high-frequency details. In this paper, we provide a set of empirical studies to confirm this limitation of pixel-based MIM and propose a new method that explicitly utilizes low-level features from shallow layers to aid pixel reconstruction. By incorporating this design into our base method, MAE, we reduce the wasted modeling capability of pixel-based MIM, improving its convergence and achieving non-trivial improvements across various downstream tasks. To the best of our knowledge, we are the first to systematically investigate multi-level feature fusion for isotropic architectures like the standard Vision Transformer (ViT). Notably, when applied to a smaller model (e.g., ViT-S), our method yields significant performance gains, such as 1.2\% on fine-tuning, 2.8\% on linear probing, and 2.6\% on semantic segmentation. Code and models are available at https://github.com/open-mmlab/mmpretrain.

==> fig/analysis.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth,scale=1.00]{pdf/analysis.pdf}
\caption{\textbf{Frequency analysis of output layer features from encoder.} Multi-level feature fusion reduces high-frequency components and enhances low-frequency components. The lowest-frequency band is labeled as \textbf{1}, while the high-frequency band is labeled as \textbf{7}.}
\label{fig:last_layer_freq}
\end{figure}


==> table/vit-s.tex <==
\begin{table}[!t]
\centering
% \scalebox{1}{
\tabcolsep 1.5pt
\begin{tabular}{lcccc}
% \toprule 
Method&Epoch&ft(\%)&lin(\%)&seg(mIoU)\\
% \midrule 
\shline
MAE&800& 78.4 & 50.5 & 41.6 \\
MFF$_\text{\tt MAE}$&800& 79.6 \more{(+1.2)} & 53.3 \more{(+2.8)} & 44.2 \more{(+2.6)}\\
MAE&1600& 78.9 & 52.3 & 42.3 \\
MFF$_\text{\tt MAE}$&1600& 80.1 \more{(+1.2)} & 54.4 \more{(+2.1)} & 44.4 \more{(+2.1)}\\
% \hdashline
% PixMIM&800& 78.3 & 49.0 & 42.0 \\
% MFF$_\text{\tt PixMIM}$&800& 79.1 \more{(+0.8)}& 54.7 \more{(+5.7)} & 43.0 \more{(+1.0)}\\
% PixMIM&1600& 78.8 & 52.3 & 42.3 \\
% MFF$_\text{\tt PixMIM}$&1600& &  & \\
\end{tabular}
% }
\vspace{-0.5em}
\caption{\textbf{Pre-train with ViT-S.}}
\label{tab:vit-s}
\end{table}

